The Nature of Ionized Gas in the Milky Way Galactic Fountain

We address the spatial scale, ionization structure, mass and metal content of gas at the Milky Way disk-halo interface detected as absorption in the foreground of seven closely-spaced, high-latitude halo blue horizontal branch stars (BHBs) with heights z = 3 - 14 kpc. We detect transitions that trace multiple ionization states (e.g. CaII, FeII, SiIV, CIV) with column densities that remain constant with height from the disk, indicating that the gas most likely lies within z < 3.4 kpc. The intermediate ionization state gas traced by CIV and SiIV is strongly correlated over the full range of transverse separations probed by our sightlines, indicating large, coherent structures greater than 1 kpc in size. The low ionization state material traced by CaII and FeII does not exhibit a correlation with either N$_{\rm HI}$ or transverse separation, implying cloudlets or clumpiness on scales less than 10 pc. We find that the observed ratio log(N_SiIV/ N_CIV), with a median value of -0.69+/-0.04, is sensitive to the total carbon content of the ionized gas under the assumption of either photoionization or collisional ionization. The only self-consistent solution for photoionized gas requires that Si be depleted onto dust by 0.35 dex relative to the solar Si/C ratio, similar to the level of Si depletion in DLAs and in the Milky Way ISM. The allowed range of values for the areal mass infall rate of warm, ionized gas at the disk-halo interface is 0.0003 < dM_gas / dtdA [M_sun kpc^-2 yr^-] < 0.006. Our data support a physical scenario in which the Milky Way is fed by complex, multiphase processes at its disk-halo interface that involve kpc-scale ionized envelopes or streams containing pc-scale, cool clumps.

==> BHBIVFitpropertiesnewhi.tex <==
 
 
\begin{deluxetable}{ccccc}
\tablewidth{0pc}
\tablecaption{BHB Intermediate Velocity Component Fits\label{tab:bhbivfits}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{BHB ID} & \colhead{Ion} & \colhead{log N$_{\rm ion}$} & \colhead{v$_{\rm LSR}$} & \colhead{$b$}}\\
\startdata
 & & & & \\
BHB1 & CaII& 11.95$\pm$0.02 &  -8.85$\pm$0.55 &  12.58$\pm$0.66 \\
&CaII& 11.30$\pm$0.04 & -29.11$\pm$0.24 &   3.87$\pm$0.36 \\
&CaII& 11.43$\pm$0.04 & -53.27$\pm$0.76 &   9.84$\pm$1.19 \\
&CaII& 11.52$\pm$0.03 & -72.30$\pm$0.30 &   5.90$\pm$0.44 \\
&FeII& 13.89$\pm$0.27 & -58.63$\pm$7.61 &  $16.20\substack{+17.42 \\ -15.20}$\\
&SiII&$<$ 14.22 & $>$-60.59 & $>$ 50.00 \\
&AlII& 12.98$\pm$0.33 & -59.41$\pm$2.89 &  10.05$\pm$7.20 \\
&SiIV& 13.35$\pm$0.04 & -61.80$\pm$2.75 &  31.39$\pm$4.18 \\
&CIV& 14.04$\pm$0.03 & -46.75$\pm$2.71 &  41.39$\pm$3.03 \\
&HI& 19.57$\pm$0.04&-19.45$\pm$1.11&  15.34$\pm$1.30\\
 & & & & \\
\hline
 & & & & \\
BHB2 & CaII& 12.56$\pm$0.01 & -28.60$\pm$0.05 &   5.86$\pm$0.06 \\
&CaII& 12.02$\pm$0.01 & -50.83$\pm$0.13 &   7.14$\pm$0.17 \\
&FeII& 14.62$\pm$0.09 & -46.07$\pm$2.42 &  15.49$\pm$3.34 \\
&SiII&$<$ 14.50 & $>$-36.40 &  22.30$\pm$21.77 \\
&AlII&$<$ 13.34 & $>$-38.84 &  25.39$\pm$24.84 \\
&SiIV& 13.26$\pm$0.04 & -46.91$\pm$3.67 &  26.27$\pm$4.37 \\
&CIV& 13.92$\pm$0.03 & -34.19$\pm$1.60 &  27.07$\pm$2.21 \\
&HI& 19.51$\pm$0.03&-38.40$\pm$0.75& 18.12$\pm$1.16\\
 & & & & \\
\hline
 & & & & \\
BHB3 & CaII& 12.14$\pm$0.02 & -23.96$\pm$0.23 &   8.20$\pm$0.37 \\
&FeII& 14.41$\pm$0.26 & -35.92$\pm$3.51 & $<$ 10.00 \\
&SiII& 14.65$\pm$0.53 & -41.45$\pm$10.73 &  17.91$\pm$14.57 \\
&AlII&$<$ 14.06 & $>$-42.09 & $<$ 10.00 \\
&SiIV& 13.58$\pm$0.02 & -61.84$\pm$2.09 &  39.11$\pm$3.07 \\
&CIV& 14.30$\pm$0.05 & -48.63$\pm$4.44 &  40.57$\pm$3.82 \\
&HI& 19.94$\pm$0.01&-12.62$\pm$0.47& 18.34$\pm$0.42\\
 & & & & \\
\hline
 & & & & \\
BHB4 & CaII& 12.25$\pm$0.01 & -17.97$\pm$0.33 &  14.36$\pm$0.49 \\
&FeII& 13.95$\pm$0.32 & -29.32$\pm$6.49 & $<$ 10.00 \\
&SiII& 14.05$\pm$0.64 & $>$-28.92 &  15.98$\pm$13.65 \\
&AlII&$<$ 13.41 & $>$-22.05 &  16.09$\pm$24.48 \\
&SiIV& 13.54$\pm$0.03 & -42.39$\pm$1.77 &  23.98$\pm$2.90 \\
&CIV& 14.27$\pm$0.03 & -24.32$\pm$1.80 &  32.37$\pm$2.05 \\
&HI& 19.73$\pm$0.02&-20.40$\pm$0.31&  11.71$\pm$0.47\\
 & & & & \\
\hline
 & & & & \\
BHB5 & CaII& 11.51$\pm$0.06 & -37.40$\pm$0.73 &   6.57$\pm$1.04 \\
&FeII& 14.12$\pm$0.12 & -42.46$\pm$4.24 &  18.75$\pm$6.56 \\
&SiII& 13.97$\pm$0.28 & -58.31$\pm$7.22 &  12.88$\pm$8.44 \\
&AlII& 13.46$\pm$0.41 & -35.50$\pm$13.82 &  28.80$\pm$6.80 \\
&SiIV& 13.38$\pm$0.03 & -68.77$\pm$2.10 &  31.21$\pm$3.18 \\
&CIV& 14.07$\pm$0.02 & -53.98$\pm$1.91 &  29.28$\pm$2.40 \\
&HI& 19.69$\pm$0.01&-14.83$\pm$1.02& 23.52$\pm$0.76\\
 & & & & \\
\hline
 & & & & \\
BHB6 & CaII& 11.98$\pm$0.06 & -31.69$\pm$0.32 &   6.59$\pm$0.55 \\
&CaII& 11.72$\pm$0.09 & -53.88$\pm$2.75 &  17.50$\pm$3.78 \\
&FeII& 13.81$\pm$0.19 & -54.75$\pm$5.47 & $<$ 10.00 \\
&SiII& 13.98$\pm$0.22 & -59.95$\pm$3.23 & $<$ 10.00 \\
&AlII& 12.97$\pm$0.69 & -61.79$\pm$5.87 & $<$ 10.00 \\
&SiIV& 13.61$\pm$0.04 & -54.30$\pm$2.46 &  34.11$\pm$2.08 \\
&CIV& 14.27$\pm$0.04 & -44.00$\pm$1.92 &  29.75$\pm$1.85 \\
&HI& 19.63$\pm$0.02&-26.95$\pm$0.52&  12.73$\pm$0.68\\
 & & & & \\
\hline
 & & & & \\
BHB7 & CaII& 11.94$\pm$0.04 & -44.74$\pm$2.12 &  21.32$\pm$0.97 \\
&FeII& 13.93$\pm$0.11 & -63.15$\pm$3.01 &  10.27$\pm$5.44 \\
&SiII& 14.66$\pm$0.06 & -35.81$\pm$2.57 &  39.64$\pm$2.23 \\
&AlII& 12.99$\pm$0.07 & -64.94$\pm$3.74 &  19.82$\pm$5.69 \\
&SiIV& 13.34$\pm$0.03 & -71.76$\pm$2.08 &  31.10$\pm$3.21 \\
&CIV& 14.10$\pm$0.02 & -53.76$\pm$1.56 &  36.50$\pm$2.26 \\
&HI& 19.52$\pm$0.03&-30.00$\pm$0.67& 16.38$\pm$1.06\\
\enddata
\tablecomments{{}  Voigt profile fit parameters for the intermediate velocity components for a variety of ionic species observed along each BHB sightline.  The parameters are: column density as log N (cm$^{-2}$), velocity centroid, v$_{\rm LSR}$ (km s$^{-1}$), and Doppler parameter, $b$, which quantifies the line width in km s$^{-1}$. We also tabulate the results from the Gaussian fits to the IV component of the HI 21-cm T$_{\rm b}$ profiles; in this case the $b$ column is given as the Gaussian $\sigma$ $\times$ $\sqrt{2}$. } 
\end{deluxetable}
 


==> BHBMWFitpropertiesnewhi.tex <==
 
 
\begin{deluxetable}{ccccc}
\tablewidth{0pc}
\tablecaption{BHB Milky Way ISM Component Fits\label{tab:bhbmwfits}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{BHB ID} & \colhead{Ion} & \colhead{log N$_{\rm ion}$} & \colhead{v$_{\rm LSR}$} & \colhead{$b$}}\\
\startdata
 & & & & \\
BHB1 & CaII& 11.48$\pm$0.06 &  -4.24$\pm$0.20 &   3.84$\pm$0.36 \\
&FeII& 14.57$\pm$0.08 & -10.30$\pm$2.27 &  16.36$\pm$3.50 \\
&SiII& 14.50$\pm$0.16 & $<$-14.24 &  35.43$\pm$3.78 \\
&AlII& 13.33$\pm$0.11 & -12.41$\pm$3.24 &  22.30$\pm$4.72 \\
&SiIV&$<$ 12.80 & $<$-14.24 & $>$ 50.00 \\
&CIV&$<$ 13.20 & $<$-14.24 &  37.06$\pm$21.44 \\
&HI& 19.97$\pm$0.01& -0.49$\pm$0.10&  8.16$\pm$0.14\\
 & & & & \\
\hline
 & & & & \\
BHB2 & CaII& 12.14$\pm$0.01 &  -2.65$\pm$0.19 &  11.64$\pm$0.28 \\
&FeII& 14.44$\pm$0.07 & $<$-12.65 &  16.48$\pm$2.73 \\
&SiII& 14.65$\pm$0.30 & $<$-12.65 &  22.33$\pm$3.86 \\
&AlII& 13.81$\pm$1.75 & $<$-12.65 &  12.83$\pm$11.73 \\
&SiIV&$<$ 12.80 & $<$-12.65 &  37.25$\pm$20.33 \\
&CIV&$<$ 13.20 & $<$-12.65 &  13.05$\pm$6.84 \\
&HI& 19.97$\pm$0.01& -2.30$\pm$0.14&  11.72$\pm$0.20\\
 & & & & \\
\hline
 & & & & \\
BHB3 & CaII& 11.89$\pm$0.00 &  -2.60$\pm$0.37 &   8.00$\pm$0.42 \\
&FeII& 14.64$\pm$0.38 & -10.39$\pm$3.57 & $<$ 10.00 \\
&SiII&$<$ 14.50 & $<$-12.60 &  23.72$\pm$5.05 \\
&AlII& 13.27$\pm$0.37 & $<$-12.60 &  15.19$\pm$8.21 \\
&SiIV&$<$ 12.80 & $<$-12.60 & $>$ 50.00 \\
&CIV& 13.42$\pm$0.34 &  -6.80$\pm$4.39 &  13.67$\pm$9.68 \\
&HI& 19.94$\pm$0.01& -1.78$\pm$0.04&  5.09$\pm$0.08\\
 & & & & \\
\hline
 & & & & \\
BHB4 & CaII& 11.25$\pm$0.08 &   1.92$\pm$0.43 &   4.38$\pm$0.67 \\
&FeII& 14.57$\pm$0.06 & $<$ -8.08 &  26.22$\pm$3.75 \\
&SiII& 14.68$\pm$0.22 &   0.85$\pm$13.57 &  38.13$\pm$7.83 \\
&AlII&$<$ 13.50 & $<$ -8.08 &  28.61$\pm$2.47 \\
&SiIV&$<$ 12.80 &  -7.06$\pm$3.81 &  12.88$\pm$7.16 \\
&CIV&$<$ 13.20 &   2.91$\pm$5.31 & $<$ 10.00 \\
&HI& 19.82$\pm$0.01& -0.90$\pm$0.11&  7.01$\pm$0.14\\
 & & & & \\
\hline
 & & & & \\
BHB5 & CaII& 11.94$\pm$0.03 &  -8.31$\pm$0.81 &  13.77$\pm$1.19 \\
&FeII&$<$ 14.80 &  -9.96$\pm$2.22 &  18.52$\pm$4.09 \\
&SiII& 15.17$\pm$0.83 & -16.57$\pm$3.84 &  15.67$\pm$6.07 \\
&AlII& 14.46$\pm$4.24 & $<$-18.31 &  13.76$\pm$18.28 \\
&SiIV&$<$ 12.80 & $<$-18.31 & $>$ 50.00 \\
&CIV&$<$ 13.20 & $<$-18.31 &  29.05$\pm$17.77 \\
&HI& 19.59$\pm$0.02& -3.91$\pm$0.19&  9.55$\pm$0.35\\
 & & & & \\
\hline
 & & & & \\
BHB6 & CaII& 11.95$\pm$0.08 & -12.74$\pm$2.89 &  19.12$\pm$3.41 \\
&FeII&$<$ 14.80 & -20.31$\pm$2.35 &  15.40$\pm$2.36 \\
&SiII& 14.85$\pm$0.24 & -18.64$\pm$3.14 &  21.21$\pm$4.44 \\
&AlII& 13.42$\pm$0.14 & -22.30$\pm$7.58 &  25.99$\pm$6.21 \\
&SiIV& 12.87$\pm$0.19 & $<$-22.74 & $<$ 10.00 \\
&CIV& 13.27$\pm$0.37 & -22.68$\pm$7.35 & $<$ 10.00 \\
&HI& 19.74$\pm$0.01& -4.15$\pm$0.28&  10.35$\pm$0.34\\
 & & & & \\
\hline
 & & & & \\
BHB7 & CaII& 11.92$\pm$0.04 &  -3.63$\pm$1.09 &  13.33$\pm$1.54 \\
&FeII& 14.73$\pm$0.12 & $<$-13.63 &  18.58$\pm$3.22 \\
&SiII& 14.85$\pm$1.16 &  -7.46$\pm$6.21 & $<$ 10.00 \\
&AlII& 15.50$\pm$0.46 & $<$-13.63 &  10.44$\pm$1.86 \\
&SiIV&$<$ 12.80 & $<$-13.63 & $>$ 50.00 \\
&CIV&$<$ 13.20 & $<$-13.63 & $>$ 50.00 \\
&HI& 19.92$\pm$0.01& -1.26$\pm$0.09&  7.78$\pm$0.13\\
\enddata
\tablecomments{{}  Voigt profile fit parameters for the Milky Way ISM
  components for a variety of ionic species observed along each BHB
  sightline.  The parameters are:  column density as log N
  (cm$^{-2}$), velocity centroid, v$_{\rm LSR}$ (km s$^{-1}$), and
  Doppler parameter, $b$, which quantifies the line width in km
  s$^{-1}$. We also tabulate the results from the Gaussian fits to the HI 21-cm T$_{\rm b}$ profiles; in this case the $b$ column is given as the Gaussian $\sigma$ $\times$ $\sqrt{2}$.  } 
\vspace{0.3in}
\end{deluxetable}
 


==> BHBproperties.tex <==
 
 
\begin{deluxetable*}{cccccccccccc}
\tablewidth{0pc}
\tablecaption{BHB Star Properties\label{tab:bhbprops}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{BHB Name, ID} & \colhead{RA} & \colhead{dec} & \colhead{$l$}  &\colhead{$b$} &\colhead{m$_{\rm FUV}$} &\colhead{m$_{\rm g}$} &\colhead{HRV} &\colhead{d} &
\colhead{x} & \colhead{y} & \colhead{z} \\
 & $(^\circ)$ &  $(^\circ)$ &  $(^\circ)$ & $(^\circ)$ &  & & (km s$^{-1}$) & (kpc) & (kpc) & (kpc) & (kpc)}
\startdata
J1527+4027 BHB1 &  231.9586 &   40.4580 &   65.6478 &   55.2262 & 16.30 & 13.78 & $-105.6$ $\pm$0.9 &   4.1 &   7.0 &  -2.1 &   3.4\\
J1534+5015 BHB2 &  233.5468 &   50.2657 &   80.9667 &   51.4485 & 16.95 & 14.20 & $-129.4$ $\pm$1.8 &   5.2 &   7.5 &  -3.2 &   4.1\\
J1344+1842 BHB3 &  206.0184 &   18.7164 &    0.8905 &   75.2642 & 17.27 & 14.46 & $-74.7$ $\pm$1.4 &   5.9 &   6.5 &   0.0 &   5.7\\
J1325+2232 BHB4 &  201.4767 &   22.5473 &    4.4384 &   80.9410 & 17.83 & 14.90 & $-100.3$ $\pm$1.8 &   7.4 &   6.8 &  -0.1 &   7.3\\
J1415+3716 BHB5 &  213.9881 &   37.2828 &   67.9148 &   69.5097 & 17.97 & 15.57 & $-134.0$ $\pm$1.2 &   9.9 &   6.7 &  -3.2 &   9.2\\
J1341+2823 BHB6 &  205.3327 &   28.3996 &   42.3913 &   78.8949 & 18.07 & 16.07 & $-124.8$ $\pm$2.2 &  11.3 &   6.4 &  -1.5 &  11.1\\
J1459+4128 BHB7 &  224.9749 &   41.4809 &   69.9352 &   60.0843 & 18.47 & 16.72 & $-183.1$ $\pm$4.4 &  15.3 &   5.4 &  -7.2 &  13.3\\
\enddata
\tablecomments{{}  Properties of target BHB stars based on SDSS DR8 SEGUE data (see Xue et al. 2011 for details); all coordinates are in epoch J2000. GALEX FUV magnitudes are determined by cross matching the closest point source detection to each BHB target.  } 
\end{deluxetable*}
 

